Multi-agent KTO: Reinforcing Strategic Interactions of Large Language Model in Language Game

Achieving Artificial General Intelligence (AGI) requires AI agents that can not only make stratigic decisions but also engage in flexible and meaningful communication. Inspired by Wittgenstein's language game theory in Philosophical Investigations, we propose that language agents can learn through in-context interaction rather than traditional multi-stage frameworks that separate decision-making from language expression. Using Werewolf, a social deduction game that tests language understanding, strategic interaction, and adaptability, we develop the Multi-agent Kahneman & Tversky's Optimization (MaKTO). MaKTO engages diverse models in extensive gameplay to generate unpaired desirable and unacceptable responses, then employs KTO to refine the model's decision-making process. In 9-player Werewolf games, MaKTO achieves a 61% average win rate across various models, outperforming GPT-4o and two-stage RL agents by relative improvements of 23.0% and 10.9%, respectively. Notably, MaKTO also demonstrates human-like performance, winning 60% against expert players and showing only 49% detectability in Turing-style blind tests.

==> Tables/ablation_makto_selfplay_old.tex <==
% sidewaystable
\begin{table}[]
    \small
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|rr|r|rrr|l}
        \toprule
         & \textbf{GPT-4o} & \textbf{Mix} & \textbf{SFT-14b} 
         & \textbf{MaKTO} 
         & \textbf{Self-play }
         & \shortstack{\textbf{w/o} \\\textbf{gameplay}}
         & \textbf{Avg. Win Rate} \\
        \midrule
        \textbf{GPT-4o} & {\color[HTML]{FF0000} 0.50} & \textbf{0.56} & 0.44 & 0.37 & \textbf{0.56} & \textbf{0.64} & 0.514 \\
        \textbf{Mix} & 0.44 & {\color[HTML]{FF0000} 0.50} & \textbf{0.58} & 0.55 & \textbf{0.71} & 0.48 & 0.553 \\
        \midrule
        \textbf{SFT-14b} & \textbf{0.56} & 0.42 & {\color[HTML]{FF0000} 0.50} & 0.48 & 0.38 & 0.66 & 0.499 \\
        \midrule
        \multicolumn{3}{l}{\textit{KTO methods}} \\
        \quad \textbf{MaKTO}-14b & \textbf{0.63} & 0.45 & \textbf{0.52} & {\color[HTML]{FF0000} 0.50} & 0.50 & \textbf{0.57} & 0.534 $(+0.04)$\\
        
        \quad \textbf{Self-play} & 0.44 & 0.29 & \textbf{0.62} & 0.50 & {\color[HTML]{FF0000} 0.50} & \textbf{0.56} & 0.483 $(-0.02)$ \\
        \quad \textbf{w/o gameplay} & 0.36 & 0.31 & 0.34 & 0.43 & 0.44 & {\color[HTML]{FF0000} 0.50} & 0.374 $(-0.13)$ \\
        \bottomrule
    \end{tabular}
    }
    \caption{Ablation study for MaKTO and other KTO training methods. \textbf{Self-play}: preference data from SFT-14B vs. SFT-14B games.  \textbf{w/o gameplay}: preference data from annotations only without actual gameplay. All models are in 14B size.}
    \label{tab:kto_vs_selfplay}
\end{table}

==> Tables/ablation_step_traj_old.tex <==
\begin{table}[h]
    \small
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|rr|r|rr|l}
        \toprule
        & & & & \multicolumn{2}{c|}{\textbf{MaKTO}} & \textbf{Avg.} \\
         & \textbf{GPT-4o} & \textbf{Mix} & \textbf{SFT-14b} 
         & \textbf{Step} 
         & \textbf{Traj}
         & \textbf{Win} \\
        \midrule
        \textbf{GPT-4o} & {\color[HTML]{FF0000} 0.50} & \textbf{0.56} & 0.44 & 0.37 & 0.45 & 0.456 \\
        \textbf{Mix} & 0.44 & {\color[HTML]{FF0000} 0.50} & \textbf{0.58} & \textbf{0.55} & \textbf{0.63} & 0.550 \\
        \midrule
        \textbf{SFT-14b} & \textbf{0.56} & 0.42 & {\color[HTML]{FF0000} 0.50} & 0.48 & \textbf{0.54} & 0.496\\
        \midrule
        \multicolumn{3}{l}{\textit{\textbf{MaKTO} with different action selections}} \\
        \quad \textbf{Step (Ours)} & \textbf{0.63} & 0.45 & \textbf{0.52} & {\color[HTML]{FF0000} 0.50} & \textbf{0.58}  & 0.545 $(+0.05)$ \\
        \quad \textbf{Traj} & \textbf{0.55} & 0.37 & 0.47 & 0.44 & {\color[HTML]{FF0000} 0.50} & 0.458 $(-0.04)$ \\
        \bottomrule
    \end{tabular}
    }
    \caption{Ablation study for MaKTO and other KTO training methods. \textbf{Stepwise}: Selecting desirable/unacceptable actions according to predefined criteria. \textbf{Trajectory}: Selecting desirable actions from winning trajectories and unacceptable actions from losing trajectories. All models are in 14B size.}
    \setlength{\tabcolsep}{4pt}
    \label{tab:traj_vs_step}
\end{table}

==> Tables/static_test_1.tex <==
\begin{table}[h!]
\centering
% \small
\resizebox{\linewidth}{!}{
    \begin{tabular}{l|rr|rr}
    \toprule
    & \textbf{Vote} & \textbf{Abstent} & \textbf{Align.} & \textbf{Wolf-pred.} \\
    & \textbf{Acc.($\uparrow$)} & \textbf{Rate($\downarrow$)} & \textbf{Acc.($\uparrow$)} & \textbf{F1($\uparrow$)} \\
    
    \midrule
    \textbf{GPT4o\_mini} & 67.2\%  & \textbf{0.4\%}          & 68.1\%            & 0.519                      \\
    \textbf{GPT4o}       & 69.4\%  & 2.3\%          & 68.0\%            & 0.587                      \\
    \textbf{Claude}      & 68.4\%  & \underline{1.0\%}          & 75.2\%            & 0.651                      \\
    \midrule
    \textbf{Qwen2.5-14b}    & 61.0\%  & 4.1\%          & 61.1\%            & 0.528                       \\
    \textbf{Qwen2.5-72b}   & 66.5\%  & 0.4\%          & 63.9\%            & 0.552                       \\
    \midrule
    \textbf{SFT-14b}     & 70.8\%  & 4.1\%          & 77.9\%            & \underline{0.712}                      \\
    \textbf{SFT-72b}     & \underline{71.1\%}  & 5.8\%          & \textbf{79.3\%}            & \textbf{0.734}           \\
    \textbf{MaKTO-72b}     &  \textbf{73.8\%}  & 1.5\%          & \underline{78.4\%}            & \textbf{0.734}   \\   
    \midrule
    \rowcolor{brown!9} \textbf{HUMAN}       & 76.7\%  & 4.8\%          & 76.1\%            & 0.742                     \\
    
    \bottomrule
    \end{tabular}
    }
    \caption{Offline results of human annotators and LLMs. The \textbf{bold} number represents the best results of the models, and the \underline{underlined} number represents the second best.}

    \label{tab:static_test}
\end{table}

==> Tables/tmp.tex <==
\begin{table}[!t]
\caption{Fine-grained behavioral analysis of SFT-72b and MaKTO-72b models against GPT-4o}
\small
\begin{tabular}{l|ccc|cc|cc|cc}
\toprule
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{General Performance} & \multicolumn{2}{c|}{Seer Role} & \multicolumn{2}{c|}{Witch Role} & \multicolumn{2}{c}{Guard Role} \\
\cmidrule{2-10}
 & Vote Acc. & Abstention & WW Check & Save & Poison & Mispoison & Protect & Misprotect & Performance↓ \\
\midrule
\multicolumn{10}{l}{\textit{As Villagers (vs GPT-4o Werewolf)}} \\
SFT-72b & 66.3\% & 6.7\% & 60.0\% & 58.0\% & 48.0\% & 38.0\% & 34.1\% & 9.5\% & - \\
MaKTO-72b & \textbf{72.7\%} & \textbf{3.2\%} & \textbf{75.7\%} & \textbf{100.0\%} & \textbf{72.0\%} & \textbf{26.0\%} & \textbf{37.6\%} & \textbf{2.3\%} & - \\
\midrule
\multicolumn{10}{l}{\textit{As Werewolves (vs GPT-4o Villagers)}} \\
SFT-72b & - & 2.2\% & 60.4\% & - & - & 32.0\% & - & 33.6\% & 32.1\% \\
MaKTO-72b & - & \textbf{4.6\%} & \textbf{57.4\%} & - & - & \textbf{48.0\%} & - & \textbf{34.7\%} & \textbf{36.2\%} \\
\bottomrule
\end{tabular}
\label{tab:fine_grain_analysis}
\end{table}
